Exploiting sparse structures and synergy designs to advance situational awareness of electrical power grid

The growing threats of uncertainties, anomalies, and cyberattacks on power grids are driving a critical need to advance situational awareness which allows system operators to form a complete and accurate picture of the present and future state. Simulation and estimation are foundational tools in this process. However, existing tools lack the robustness and efficiency required to achieve the level of situational awareness needed for the ever-evolving threat landscape. Industry-standard (steady-state) simulators are not robust to blackouts, often leading to non-converging or non-actionable results. Estimation tools lack robustness to anomalous data, returning erroneous system states. Efficiency is the other major concern as nonlinearities and scalability issues make large systems slow to converge. This thesis addresses robustness and efficiency gaps through a dual-fold contribution. We first address the inherent limitations in the existing physics-based and data-driven worlds; and then transcend the boundaries of conventional algorithmic design in the direction of a new paradigm -- Physics-ML Synergy -- which integrates the strengths of the two worlds. Our approaches are built on circuit formulation which provides a unified framework that applies to both transmission and distribution. Sparse optimization acts as the key enabler to make these tools intrinsically robust and immune to random threats, pinpointing dominant sources of (random) blackouts and data errors. Further, we explore sparsity-exploiting optimizations to develop lightweight ML models whose prediction and detection capabilities are a complement to physics-based tools; and whose lightweight designs advance generalization and scalability. Finally, Physics-ML Synergy brings robustness and efficiency further against targeted cyberthreats, by interconnecting our physics-based tools with lightweight ML.

==> overview.tex <==

Chapter 2:

\section{Simulation and estimation key to situation awareness} \label{sec: intro SA}

Situation awareness (SA) \cite{SA_overview} means the operator’s understanding and perception of the dynamic situation. The concept is initially defined by Tolk and Keether in the aircraft domain: “the ability to envision the current and future disposition of both red and blue aircraft and surface threats''. Endsley extended the early definition beyond fighter aircraft while still highlighting the \textbf{"present and future"}. The understanding of SA is also advanced by the operational methods and performance measures defined to evaluate the operator’s SA. Examples include the situation awareness rating technique (SART) and the SA global assessment technique (SAGAT). 

This thesis discusses steady-state situation awareness in the context of the power grid as a characteristic of operators under the changing grid conditions. It refers to grid operator's ability to perceive and understand the system’s \textbf{present} state and project its \textbf{future} behavior. Present situation awareness provides operators with a real-time snapshot of system conditions, while future situation awareness enables them to anticipate potential challenges and make proactive decisions.

Estimation (and detection) tools are fundamental for present situation awareness which focuses on providing a real-time snapshot of system conditions for real-time understanding of the current conditions. This involves recognizing current power flows, voltages, equipment status, and any ongoing disturbances based on real-time data (e.g., through state estimation). And the goal is to provide operators with an accurate and up-to-date representation of the system's status, allowing them to maintain control and respond to current issues. Below we informally define the estimation problem for present situation awareness. For a comprehensive understanding of the present operating conditions, estimation problem needs to go beyond the estimating states of the system, but also ongoing anomalies:

\begin{problem}[Power grid estimation for present  situation awareness]\label{def-informal:estimation} \noindent\\
\textbf{Input:} network parameters and real-time measurement data at time $t$;
measurement models depicting how data relates to the variables to estimate; 
(optional) historical data at time $1, ..., t-1$, (optional) past events and switching history.\\
\noindent\textbf{Output (for time $t$):} estimated system state variables (typically bus voltages which can be further used to calculate line currents, and power flows), updated topology (an accurate view of the network connectivity), and anomaly alerts 
\end{problem}

Simulation is the fundamental tools for future situation awareness which is to anticipate and project potential future states of the system based on current and forecasted conditions. This could include answering "what-if" questions on how the system states will evolve under changing loads, equipment failures, or other contingencies. The goal here is to help operators foresee whether the system can survive changes and serving current or forecasted loads, so that they can foresee potential risks and prepare for them in advance to ensure system reliability. Below we informally define the simulation problem for future situation awareness of power grid:

\begin{problem}[Power grid simulation for future steady-state situation awareness]\label{def-informal:simulation}  \noindent\\
\textbf{Input:} the state at time $t_1$ (e.g., obtained from estimation), possible "what-if" scenarios for a future time $t_2$ (e.g., changes in load, generation forecasts, equipment failures, other contingencies, etc.), and system models in the form of network balance equations.\\
\noindent\textbf{Output (for future time $t_2$):} system behavior (typically bus voltages which can be used to further calculate currents, power flows, etc)  
\end{problem}

The goal of this thesis is to build high-quality situation awareness to handle a variety of threats, ranging from physical to cyber indents;  from natural faults to malicious attacks; and from random perturbations to targeted or interactive threat behaviors. Table \ref{tab: threats} summarizes threats that represent key obstacles in power system situation awareness. 

\textbf{Cyber attacks on power grid:} Cyberattacks are of particularly high interest in this case. Recent years have witnessed and documented a large variety of cyber attack methods capable of causing different consequences. Some de-energize the power grid in a brute-force way via intrusion into the substation, power plants or control rooms to open circuit breakers  (e.g., power outage in 2015\cite{ukrain2015} and 2016 Ukrainian attacks\cite{lee2017crashoverride}). Some target IoT-controlled load devices on the distribution grid for a manipulation of demand to destabilize the power grid (e.g., MadIoT attack\cite{madiot}\cite{MadIoTRebuttal}\cite{MadIoTOnNY}). Some aim at data loss and delay by attacking the communication channels (e.g., jitter attack\cite{jitter_attack}). And some inject targeted false data to mislead the operators (e.g. false data injection attack\cite{FDIA_AC}\cite{fdia-acse}). Unlike traditional bad data, false data generated by a cyber attack are usually assumed to be targeted and interactive, meaning they are inter-correlated or even carefully designed by some relationship to maximize the impact. 

Being aware of these threats, advanced situation awareness tools are needed to defend against them. Real-time estimation needs to identify data errors and maintain "present" situation awareness regardless of them. Whereas for threats on physical layer, advanced simulation tools are needed to proactively simulate contingencies and blackouts, so as to gain future situation awareness of potential failures and build resiliency against them.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Threats that represent key obstacles in power system situation awareness}
\label{tab: threats}
\begin{tabular}{l|l|l}
\hline
\textbf{type}                                     & \textbf{threat}                                                                                              & \textbf{possible causes}                                                                                                           \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{traditional}} & \begin{tabular}[c]{@{}l@{}}random data error \\ and low data quality\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}large measurement noise, meter mis-calibration, \\ communication error, etc\end{tabular}                \\ \cline{2-3} 
\multicolumn{1}{c|}{}                             & \begin{tabular}[c]{@{}l@{}}topology error \\ (wrong switch status data)\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}circuit breaker fault, communication error or latency, \\ switch data mis-synchronization\end{tabular}  \\ \cline{2-3} 
\multicolumn{1}{c|}{}                             & \begin{tabular}[c]{@{}l@{}}traditional contingency \\ (outage of \\ generator/line/transformer)\end{tabular} & \begin{tabular}[c]{@{}l@{}}overloading, physical damage,  mechanical issues,\\ circuit breaker faults, etc\end{tabular}            \\ \cline{2-3} 
\multicolumn{1}{c|}{}                             & blackout                                                                                                     & high demand conditions, (cascading) contingencies                                                                                  \\ \hline
\multirow{3}{*}{modern}                           & \begin{tabular}[c]{@{}l@{}}interactive data errors \\ induced by cyber attacks\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}cyber intrusion into meters / communication / data center \\ to inject false data, \\jamming / spoofing attacks on modern synchrophasors, etc \end{tabular}          \\ \cline{2-3} 
                                                  & supply / load purtabations                                                                                   & MadIoT attack, renewable energy variations, etc.                                                                                   \\ \cline{2-3} 
                                                  & \begin{tabular}[c]{@{}l@{}}contingency and blackout\\ induced by cyberattacks\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}cyber intrusion into substations / power plants / \\ control room to disconnect generators, etc\end{tabular} \\ \hline
\end{tabular}
\end{table}



\section{Robustness and efficiency gaps}
%\reminder{here first talk about overall description and meaning of robustness and efficiency troubles}
 
The word "robustness" has many connotations in different fields. This thesis discusses the lack of robustness in simulation and estimation tools, meaning that, under some threat conditions, they result in erroneous, meaningless outputs or even cannot reach a solution. In the rest of this Chapter, Section \ref{sec: simulation gap} discusses existing simulation methods and their lacking robustness to blackout failures; and Section \ref{sec: estimation gap} discusses the existing estimation approaches and their limited robustness to realistic set of data errors. 

Whereas, the efficiency gap refers to the lack of time-efficiency in existing tools. The challenge stems from the nonlinearity introduced by analytical models, specifically nonlinear network models in simulation, and nonlinear measurement models in estimation, respectively. These nonlinear models result in nonlinear programming problems that are NP-hard and large systems are slow to converge especially when the solver does not have a good initial point to start with.

Next in Section \ref{sec: simulation gap} and  \ref{sec: estimation gap}, we will go through the robustness and efficiency gaps in each tool, with a review of traditional and state-of-the-art approaches in literature. 

\subsection{Gaps in (steady-state) simulation tools}\label{sec: simulation gap}
\subsubsection{Traditional power flow simulation}
Simulation evaluates whether a system can survive "what-if" scenarios while serving current or forecasted loads. Traditional method for this purpose outputs the bus voltage solution by iteratively solving a set of nonlinear network balance equations. Let $ N_{bus}$  be the number of buses (nodes), $ V_i $ be the voltage magnitude at bus $ i $, $ \theta_i $ be the voltage phase angle at bus $ i $, 
\( P_{G_i} \) be the active power supply generated at bus \( i \), \( P_{\text{load}_i} \) be the active power consumed by the load at bus \( i \), \( Q_{G_i} \) be the reactive power generated at bus \( i \), \( Q_{\text{load}_i} \) be the reactive power consumed by the load at bus \( i \).
%$ P_i $ is the active power injected at bus $ i $, $ Q_i $ is the reactive power injected at bus $ i $, 
$ Y_{ij} = G_{ij} + jB_{ij} $ be the element of the admittance matrix $ Y $, where $ G_{ij} $ and $ B_{ij} $ are the conductance and susceptance between buses $ i $ and $ j $, respectively. Each node $i$ is constrained by two network equations in (\ref{eq:powerbalance}) that enforce power balance for both the active (real) and reactive (imaginary) components of the power. They intuitively mean that the total amount of power flowing into the bus must equal the total amount of power flowing out of the bus.
\begin{align} 
F_i(V, \theta) =
\begin{cases}
P_{G_i} - P_{\text{load}_i} - V_i \sum_{j=1}^{N} V_j \left( G_{ij} \cos(\theta_i - \theta_j) + B_{ij} \sin(\theta_i - \theta_j) \right) = 0 \\
Q_{G_i} - Q_{\text{load}_i} - V_i \sum_{j=1}^{N} V_j \left( G_{ij} \sin(\theta_i - \theta_j) - B_{ij} \cos(\theta_i - \theta_j) \right) = 0 
\end{cases}
\label{eq:powerbalance}
\end{align}

So the traditional power flow simulation problem can be mathematically defined as:

\begin{problem}[Traditional power flow simulation]\label{def: trad simulation} evaluates "what-if" scenarios by solving bus voltage solution $V, \theta$ from a set of nonlinear equations: 
\begin{equation}
    F_i(V, \theta)=0 \text{ as in  (\ref{eq:powerbalance}), for }  i=1,2,...,N_{bus} 
\end{equation}
\end{problem}
Such a traditional power flow simulation aims to converge to a so-called "feasible" solution of the system. The efficiency gap arises in the process of reaching convergence, as the nonlinear function $F$ makes it a nonlinear programming problem that is generally considered NP-hard. Newton-Raphson method is the common method to solve it where the nonlinear equations are linearized iteratively, and solutions are updated until convergence. But there is no general guarantee that all instances can be solved efficiently, particularly for large and complex networks.

And this traditional method fails completely if no feasible solution exists for the system, which represents the scenario of power system blackout. Often, due to severe contingencies, heavy loading, and other limitations that make power supply unable to meet the demand, simulation indicates network collapse, which corresponds to a grid that has likely blacked out \cite{powerblackout}. What-if scenarios related to blackouts are of high interest to both operation and planning, since they result in severe consequences ranging from economic loss, physical damage of infrastructure, and severe social disruptions. 

Traditional method is not robust to such failures. In  Problem Definition \ref{def: trad simulation} formulation, this collapsed grid state mathematically represents an "infeasible system" with no solution exists to the equations $F(V, \theta)=0$. The methodology diverges \cite{powerflow-diverge}, resulting in no useful information from the simulation output. 

\subsubsection{Infeasibility-quantified simulation to converge under blackouts}
To avoid divergence without providing information, improved simulation method \cite{SUGAR-pf-marko},\cite{infeasibility-quantified-pf-trad},\cite{SUGAR-pf} has been developed to provide meaningful power flow solutions for such collapsed grid states. The main idea is to quantify the "infeasibility" of these traditionally unsolvable cases and reformulating simulation into a constrained optimization problem:


\begin{problem}
[Infeasibility-quantified simulation]\label{def: sugar simulation} evaluates "what-if" scenarios while considering possible blackouts by solving $x=[V, \theta]$ and compensation terms $n$ from: 
\begin{align}
&\min_{x,n} \frac{1}{2}||n||_2^2\notag\\
\text{s.t. }
   & F_i(x)+n_i=0 \text{ for }  i=1,2,...,N_{bus} 
\end{align}
\end{problem}


\noindent Specifically, this new formulation introduces additional slack variables $n_i$ at each bus $i$ with intuitive meanings:
\begin{itemize}
    \item $n_i$ is a "infeasibility" indicator" that indicates power deficiency at each location that causes system blackout
    \item $n_i$ also represents compensation terms that capture how much additional flow needs to be injected at each bus to make the network balance conditions hold again
\end{itemize}
\noindent So that at each bus $i$, the traditional system model $F_i(x)=0$ with $x=[V,\theta]$ can be extended to a new set of equations $F_i(x)+n_i=0$. This modified system with compensations mathematically represents a feasible system with infinite solutions. By minimizing the sum of squares (i.e., L2 norm) of the compensation terms, the method reaches the optimal solution that minimizes the "energy of reconstruction error", considering $n$ as the error that prevents the system from being feasible. 

The variables $n$ are "infeasibility indicators" which extend traditional simulation to account for both feasible and infeasible systems. The values of $n$ can clearly identify a feasible case from an infeasible one. Convergence with zero $n$ everywhere denotes system balance satisfied and feasible solutions reached. Convergence with nonzero $n_i$ at any node $i$ denotes an infeasible system with specific power flow deficiency at each bus $i$. Whenever, divergence happends, it is totally due to insufficient convergence techniques of the algorithm.

Such "infeasibility-quantified" simulation has been proposed and developed for both the traditional power flow simulation \cite{infeasibility-quantified-pf-trad} which models power balance as in (\ref{eq:powerbalance}), and newer circuit formulations of power system \cite{SUGAR-pf-marko}\cite{SUGAR-pf} which models current balance under rectangular coordinate, the later allows application to three-phase distribution grid without loss of generality \cite{SUGAR-pf}.

\subsection{Gaps in estimation (and detection) tools} \label{sec: estimation gap}

\subsubsection{Estimation input: conventional and modern data}

As informally defined in Problem \ref{def-informal:estimation}, the the "present" situation awareness aims to retrieve real-time system information from measurement data. These data come from a large number of meters, i.e., sensors, installed across the system. These meters collect measurements over time on different types of buses and branches (transmission lines and transformers). The type and quality of measurement data depends highly on the type of measurement device. Table \ref{tab: data collection} shows the realistic setting of data collection with a detailed comparison.

Conventional monitoring technologies, like the supervisory control and data acquisition (SCADA) system, collect steady-state measurements of circuit-breaker status (or switch status), voltage magnitude $|V|$, current magnitude $|I|$, real and reactive power flows $P,Q$. These data usually have the measurement accuracy of $\pm 2\%$ as required by PJM\cite{pjm-m01}. 
Remote terminal units (RTU), also called remote telemetry units, act as the interface in the SCADA system to gather all data from field devices and transmit them to the master station in a central control system. Any control signal issued by the control center will also be received by RTU and further delivered to the field devices (e.g., relays). In this work, we use RTU to represent the measurement device in SCADA. 

Modern networked phasor measurement units (PMU) collect voltage and current phasors, frequency, etc, with high speed and accuracy. The transient data measured by PMUs are synchronized by the Global Positioning System (GPS) and transferred to the control center via a hierarchy of local and regional phasor data concentrators (PDCs) as well as the underlying synchrophasor communication networks (ranging from wired to wireless networks). A review of PMU communication technologies can be found in \cite{review-pmu-tech}.
Unlike the magnitude signals collected by conventional SCADA, synchrophasors are characterized by both the real-time magnitude and phase angle of an electrical phasor quantity (voltage or current). Each phase angle is with respect to a consistent reference across the system, whereas SCADA data only enable computing a local phase angle between voltage and current. 
Usually, PMU is more than 100 times faster than the conventional SCADA system, with a sampling rate of over 600Hz, a reporting rate of more than 30 samples per second, and an accuracy of $\pm 1\%$ or better for all measurements.
The last decade has seen PMUs installed on both the transmission and distribution grid (distribution-level PMU, micro-PMU or $\mu$PMU on distribution grid), allowing for real-time transient monitoring, data analysis and operation. Today's industrial practices and guidelines\cite{pmu_guideline} require that PMUs be placed near significant generating plants generally above 100 MVA (including wind and solar), large load buses, and grid control devices to capture safety-critical incidents. Reports\cite{pmu_coverage2019} showed the number of PMU deployment in the US grid bulk power system (i.e., the generation and transmission system) was over 2,500 in 2019 and over 3,000 in 2022. 

\begin{table}[]
\caption{Realistic settings of data collection on power grid}
\label{tab: data collection}
\small
\begin{tabular}{llllll}
\hline
\multicolumn{1}{c|}{\textbf{location}}                                                                          & \multicolumn{1}{c|}{\textbf{device}}                                              & \multicolumn{1}{c|}{\textbf{data}}                                                                                                                               & \multicolumn{1}{c|}{\textbf{type}}                                                & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}frequency of \\ acquisition\end{tabular}}}     & \multicolumn{1}{c}{\textbf{accuracy}}                                                    \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}transmission\\ and\\ distribution\end{tabular}}} & \multicolumn{1}{l|}{RTU}                                                          & \multicolumn{1}{l|}{switch status}                                                                                                                               & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}discrete \\ (on/off)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}upon change in PJM,\\ every 4 seconds in\\ ISO-NE\end{tabular}} & \multicolumn{1}{c}{-}                                                                    \\ \cline{2-6} 
\multicolumn{1}{l|}{}                                                                                           & \multicolumn{1}{l|}{RTU}                                                          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}voltage/current magnitude,\\ real/reactive power,\\ frequency\end{tabular}}                                       & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}analog\\steady-state\end{tabular}}                                                 & \multicolumn{1}{l|}{2-10 seconds}                                                                     & \begin{tabular}[c]{@{}l@{}}$\pm2\%$\\ in PJM\end{tabular}                                \\ \hline
\multicolumn{1}{l|}{transmission}                                                                               & \multicolumn{1}{l|}{PMU}                                                          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}voltage/current phasor,\\ frequency,\\ rate of change of frequency,\\ dynamic reactive device power\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}analog\\transient\end{tabular}}                                                    & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}reporting rate $\geq$ 30\\ samples/second\end{tabular}}  & \begin{tabular}[c]{@{}l@{}}$\pm 1\%$\\ (angle $\pm1\degree$ \\ or $\pm1\%$)\end{tabular} \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{distribution}}                                                              & \multicolumn{1}{l|}{$\mu$PMU}                                                    & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}voltage/current phasor,\\ frequency, etc\end{tabular}}                                                            & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}analog\\transient\end{tabular}}                                                   & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}reporting rate 10-120 \\samples/second\end{tabular}}     & \begin{tabular}[c]{@{}l@{}}$\pm1\degree$ \\ or $\pm1\%$\end{tabular}                     \\ \cline{2-6} 
\multicolumn{1}{l|}{}                                                                                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}smart meter, \\ IoTs\end{tabular}} & \multicolumn{1}{l|}{loads, line flows, etc}                                                                                                                      & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}analog\\steady-state\end{tabular}}                                                 & \multicolumn{1}{c|}{-}                                                                                & \multicolumn{1}{c}{-}                                                                    \\ \hline
\multicolumn{6}{l}{\begin{tabular}[x]{@{}l@{}}
* This table mainly includes regular electronic updates. Some significant events like changes in transformer tap \\position, dynamic ratings are not included (more details in \cite{pjm-m01}. But the real-world control room will be notified \\immediately upon these events. \\
* RTUs and PMUs provide measurements for buses, transmission lines, transformers and reactive devices (like\\ synchronous condensers).
\end{tabular}}                                       \end{tabular}
\end{table}

\textbf{Observability issues and pseudo-measurements}: The transmission system requires collected measurements to guarantee system observability. The concept of observability was initially defined by F. Schweppe and Wildes in \cite{WLS-SE} as being able to uniquely determine all the state variables (bus voltage magnitudes and phase angles) from the given set of measurements using the control room's state estimation (SE) algorithm. This requires proper meter placement depending on the type, location and number of measurements. However, in real-time operation, a temporary unavailability of data might occur and cause an unobservable system or unobservable islands. In this case, we can add pseudo-measurements which will be handled the same way as real data in the estimation problem. These measurements can be nominal load/generation settings, estimated coefficients or patterns such as the daily load cycle, zero-injection buses, etc. 

Taking these measurements as input, the estimation task for present situation awareness (as informally defined in Problem \ref{def-informal:estimation}) is traditionally split into 3 processes: 1) network topology processor for topology estimation, 2) state estimator (SE) for estimating state variables (voltages), and 3) bad data detection which is typically implemented by hypothesis tests immediately after the state estimation. Later methods of robust state estimation merges 2) and 3) together into one unit. And generalized state estimation (GSE) merges 1) and 2) together to jointly estimate topology and voltages. And a robust version of GSE merges 1), 2) and 3) together into one. Next we will discuss existing methods in terms of their formulations and limitations. In general, the inclusion of traditional is the main source of nonlinearity and that results in efficiency challenges to estimation. And the random and targeted data errors, as illustrated in Table \ref{tab: threats}, results in the gap of robustness. 

\subsubsection{Network Topology Processor} \label{sec: NTP}

 A network topology processor provides situation awareness of the network topology.   In today's control room, NTP converts the NB model into a simplified bus-branch (BB) format to be used by state estimation, contingency analysis and optimal control. As Figure \ref{fig: NB to BB} shows, the node-breaker (NB) model includes all inactive and active switch components that exist on the system, whereas the bus-branch model only contains active bus and branch components which significantly decrease the size of the network. 

  \begin{figure}[h]
  \begin{subfigure}[t]{0.53\textwidth}
      \centering	\includegraphics[width=\textwidth]{figures/reality/NB_model.png}
	\caption{Node-breaker (NB) model of a grid sub-network.}
	\label{fig:NB model}
  \end{subfigure}
  \hfill
    \begin{subfigure}[t]{0.43\textwidth}
      	\centering	\includegraphics[width=\textwidth]{figures/reality/BB_model.png}
	\caption{Bus-branch (BB) model: substation buses are merged.}
	\label{fig:BB model}
    \end{subfigure}
    \caption{Network topology processor converts node-breaker (NB) model is to bus-branch (BB) model, and identifies network topology.}
    \label{fig: NB to BB}
  \end{figure}

 
 The standard algorithm for NTP is as follows:
\begin{enumerate}
    \item \textit{Raw data processing} converts raw data into normalized units and performs simple checks to verify operating limits, rate of change of operating variables, and other data consistency checks (e.g., confirm zero flows on open switches and zero voltage across closed switches).
    \item \textit{Bus section processing} recursively merges any two nodes connected by a closed switch into one bus.
    \item \textit{Connectivity analysis} identifies active network topology from the switch status data and reassigns locations of metering devices on the bus-branch model.% Energized islands and the equipment-to-bus correspondence are also identified within this step.
\end{enumerate}
As only minor or no topology changes occur most of the time between subsequent NTP runs, a real-world NTP increases its efficiency by operating in tracking mode where only the groups of bus sections with switch status changes are processed recursively. 

When processing on the NB model, NTP assumes all its input status data are correct. However, switch status data  can be corrupted due to telemetry error, operator entry error, physical damage (e.g., a line is tripped but the disconnection is not reflected on the circuit breaker status) or even a cyber-attack. In case of such incorrect statuses, NTP can falsely merge/split buses and output an erroneous grid topology. 

\subsubsection{State estimation and bad data detection}\label{sec: SE}

Taking the network topology and measurement data as input, 
grid operators run AC state estimation (ACSE) at minute scale (every 5 minutes in ERCOT and US Midwest ISO (MISO), every 3 minutes in the U.K. grid and ISO-NE, and every 1-2 minutes in PJM\cite{pjm-m12}) to gain situational awareness of the AC grid state variables and bad data alarms.
The AC state variables include voltage magnitude and phase angle at every bus. They are used to estimate the generation and load configurations together with network topology and parameters, to provide situation awareness of the up-to-date AC power flow model (i.e., system model description) to be used in contingency analysis, optimal power flow and other studies. 

Traditional method  \cite{WLS-SE} for this purpose is a weighted least squares (WLS) method:

\begin{problem}[Traditional AC state estimation]\label{def: trad SE} Given a vector of measurement $z$, state estimation solves  bus voltages $x=[|V|,\theta]$ by minimizing the weighted least-squares (WLS) of measurement error:
    \begin{equation}
    \min_x \sum_i w_i(z_i-f_i(x))^2
    \label{eq: trad SE}
    \end{equation}
\end{problem}

\noindent where $x$ is the vector of state variables containing  voltage magnitudes $|V|$ and phase angles $\theta$, $z_i$ is the $i$-th measurement, and $f_i(x)$ denotes the relationship between measurement $z_i$ and state $x$. 

The function $f_i(x)$ for $\forall i$ is determined by Kirchoff’s law and power flow equations. The efficiency gap arises as $f_i(x)$ is a nonlinear equation for some conventional SCADA measurements like the real and reactive power, e.g.,
\begin{equation}
    P_{i}  = V_i \sum_{j=1}^{N} V_j \left( G_{ij} \cos(\theta_i - \theta_j) + B_{ij} \sin(\theta_i - \theta_j) \right) 
\end{equation}

\noindent making the objective function nonlinear and non-convex. Thus, this minimization problem does not have a closed-form solution and must be solved iteratively. 

The robustness gap also arises when facing data errors as listed in Table \ref{tab: threats}. 
The most classical family of methods to figure out bad data are hypothesis tests based on post-processing of the weighted least square (WLS) problem residuals \cite{traditional-BDI},\cite{robustSE-reweight},\cite{robustSE-modify}. More specifically:
\begin{problem}[Traditional bad data detection (BDD)]\label{trad BDD}
    Assuming that the measurement noise satisfy Gaussian distribution, the WLS residual $J_i=(z_i-f_i(\hat{x}))^2, \forall i$ (obtained from traditional state estimation Problem \ref{def: trad SE}) satisfies Chi-square distribution whose critical value $\tau$ can be used as a threshold to detect bad data.
    \begin{equation}
        z_i \text{ is a bad data if } J_i>\tau
    \end{equation}
\end{problem}
 Based on hypothesis testing, bad data is usually handled by adjusting suspicious measurements and rerunning ACSE until residuals are satisfactory. Possible adjustments include removing bad data, modifying \cite{robustSE-modify} bad data or the iterative reweighted least square method \cite{robustSE-reweight}, where weights on suspicious measurements are set to lower values. Clearly, the iterative re-running of the ACSE problem incurs a computational burden. Other robust estimators include least median of squares \cite{robustSE-median}, yet this is not widely adopted due to numerical difficulty in handling the median.

The family of \textbf{robust state estimators} has been developed as the performance of residual-based hypothesis tests can be unsatisfactory, especially when multiple bad-data exist. Built upon the assumption that bad data are typically sparse, the problem formulation is typically based on minimizing the weighted least absolute value (WLAV) in the objective function \cite{LAVSE-dc-soliman}\cite{LAVSE-dc-Vidya}\cite{LAVSE-PMU-abur}\cite{LAVSE-PMU-abur2}. These methods 
%make use of the nice property that "minimizing L1 norm of a vector induces its sparsity", to 
enable automatic rejection of bad data, eliminating the need for iterative re-runs while providing clear identification of suspicious measurements from the sparse residual vector:
\begin{problem}[Robust state estimation]\label{def: trad SE} Given a vector of measurement $z$, robust SE solves  bus voltages $x=[|V|,\theta]$ by minimizing the weighted least absolute value (WLAV) of measurement error, resulting in a sparse residual to capture and reject (random) bad data:
    \begin{equation}
    \min_x \sum_i w_i|z_i-f_i(x)|
    \label{eq: WLAV SE}
    \end{equation}
\end{problem}



Despite this desirable property, the non-differentiable L1-norm terms in the WLAV approach introduces additional complexity. At present, two approaches to WLAV-ACSE exist: i) those that solve highly non-convex ACSE due to inclusion of power measurements from conventional RTUs \cite{LAVSE-dc-Singh-splitform}; and ii) those that are formulated as a linear programming (LP) problem \cite{LAVSE-PMU-abur}\cite{LAVSE-PMU-abur2} with the assumption that network only consists of PMUs. These convex WLAV formulations based solely on PMUs take advantage of the linear relationship between phasor data and grid states; however, assuming PMU-observability of the network is unrealistic for grids today. And Simplex method\cite{simplex}, which is typically used to solve linear programming problems in these linear SE tasks, is not scalable to large systems.

To be practical for the reality, ACSE must include RTUs (i.e., conventional SCADA measurements). Unfortunately, most methods that include conventional RTUs (hybrid or otherwise) correspond to ACSE methods with highly complex and non-convex solution space that presents convergence challenges and high residuals. To address these problems, there has been some work on convex relaxations of ACSE methods (applicable to WLAV as well). For instance, \cite{convexTESE-SDP-weng} convexified the problem by reformulating the voltage magnitude $|V|$, phase angle $\delta$, and product of $V$ and $I$, in semidefinite programming (SDP) form, through matrix transformation; however this method fails to effectively scale  to large-scale networks. More recently to overcome the convergence and high residual limitations, the researchers in \cite{SUGAR_SE_L2}\cite{SUGAR-SE-Alex} proposed a circuit theoretic ACSE approach that reduces the problem to an equality-constrained quadratic programming (QP) problem by creating linear measurement models following a "sensitivity" based mapping of conventional grid measurements. This approach provides a convex hybrid ACSE formulation scalable to large networks, but it is not implicitly resilient to bad data.

\subsubsection{Generalized State Estimation} \label{sec: GSE}

Despite with a simple checking of data consistency, NTP does not include a rigorous analysis to correct wrong switch statuses. Thus, NTP's topology output can be inaccurate. The SE, which takes the erroneous topology as input, always assumes the given topology is correct and the bad-data detection algorithms cannot separate bad data from topology errors. Thus, any topology error will harm the operator's situation awareness by falsifying the SE solution while remaining undetectable. 

There have been attempts to build robustness against wrong switch statuses and resulting topology errors\cite{TE-GSE}\cite{TE-WLSE-BDI}\cite{TESE-GSE-PMUabur}\cite{convexTESE-SDP-weng}. One approach is a variant of ACSE bad-data detection (BDD) \cite{TE-WLSE-BDI} which runs ACSE for a set of possible topologies and then determines the optimal topology based on the one with the smallest residual. However, the problem becomes combinatorial and expensive to solve when multiple wrong switch statuses exist.

A more solvable family of methods is generalized state estimation (GSE), also known as generalized topology processing. The classical generalized state estimation (GSE)\cite{TE-GSE} was demonstrated on a small substation network using a linear DC grid model with node-breaker representation. The algorithm is as follows:
\begin{enumerate}
    \item \textit{Switch modeling}: For any switch $(sw)$ that connects node $i,j$ in the NB model, \cite{TE-GSE} creates a pseudo measurement of zero power flow ($P_{ij}=0$) if it is open, and zero angle difference ($\theta_{ij}=0$) if it is closed. Other elements are modeled similarly to the bus-branch model.
    \item \textit{Estimation}: These pseudo measurements for discrete states, along with the analog measurements, are then used to run state estimation on the network.
    \item \textit{Bad data detection}: A hypothesis test is performed on the residual of each switch and analog measurement to check if any data value is wrong. 
\end{enumerate}
 While a DC model \cite{TE-GSE} provides the desirable properties of linearity and problem convexity, it does not have the expressiveness or fidelity to represent the AC system accurately. Therefore, \cite{GSE-AC-nonlinear} extended the DC-GSE \cite{TE-GSE} to AC-network constrained GSE. But this presents challenges as well. Due to nonlinear branch flow equations, AC-GSE results in a non-convex formulation with significant drawbacks in performance \cite{GSE-AC-nonlinear}. More recently, advanced GSE methods \cite{TESE-GSE-PMUabur}\cite{convexTESE-SDP-weng}\cite{TESE-GSE} have applied WLAV method on node breaker (NB) model to perform the joint estimation of AC states and topology for the entire AC power grid, allowing traditional bad data and topology errors to be effectively identified and separated. Below gives a general formulation of these approaches:
 
 \begin{problem}[Robust generalized state estimation]\label{def: trad SE} Given a vector of continues measurement $z_{cont}$ and a vector of switch statuses $s$, GSE defines slack variables $y_{i,j}$ representing (current or power) flow on each switching device $(i,j)$, and crease pseudo measurements $z_{sw}$ according to its measured status. Then solve bus voltages $x=[|V|,\theta]$ and flows $y$ from an extended measurement vector $z=[z_{cont},z_{sw}]$ by minimizing the weighted least absolute value (WLAV) of measurement error, resulting in a sparse residual to capture and reject (random) bad data:
    \begin{equation}
    \min_{x,y} \sum_i w_i|z_i-f_i(x)-M_i\cdot y|
    \label{eq: WLAV SE}
    \end{equation}
\end{problem}

 
However, due to possible nonlinear $f_i$ functions, similar drawbacks as in robust state estimation also limit the time-efficiency of GSE approaches. \cite{TESE-GSE-PMUabur} assumed full observability of the network model using PMU data alone, so that $f_i$ functions are linear, but the assumption remains unrealistic in most countries and regions where traditional SCADA RTU meters are still dominant.  \cite{convexTESE-SDP-weng} used semidefinite programming (SDP) relaxation to obtain a convex GSE formulation, but SDP does not scale well to large-scale systems \cite{large-scale-SDP}. 



\subsection{Data-driven learning-based situation awareness tools}


\subsubsection{Function approximators of simulation and estimation}

Finding data-driven alternatives to physics-based simulators or estimators has widely studied in recent years. The common strategy is to leverage neural networks to approximate the physical functions in power system analysis. The application includes not only power flow (PF) \cite{ppf-dnn}\cite{pf-dnn-topo}\cite{gnn-pf} and state estimation (SE) \cite{unrolled-se-2018}\cite{unrolled-se}\cite{unrolled-gnu-se}, but also optimal power flow problems, ranging from DC optimal power flow (DCOPF)\cite{dcopf-dnn} to ACOPF \cite{acopf-dnn-donti}\cite{gnn-acopf}\cite{gnn-acopf-warm}. 

These methods are generally based on (usually supervised) learning of the input-to-solution mapping using historical system operational data or synthetic data. 
A popular type of method is to learn a 'one-step' mapping function. Some use deep neural network (DNN) architectures \cite{ppf-dnn}\cite{pf-dnn-topo}\cite{acopf-dnn-donti}\cite{dcopf-dnn} to learn high-dimensional input-output mappings, some use recurrent neural nets (RNNs) \cite{rnn-dse} to capture grid dynamics, and others apply graph neural networks (GNN) \cite{gnn-pf}\cite{gnn-acopf}\cite{gnn-se} to capture the exact topological structure of power grid. One the other hand, another type of method particularly designed for state estimation tasks is unrolled neural networks \cite{unrolled-se-2018}\cite{unrolled-se}\cite{unrolled-gnu-se}, whose layers mimic the iterative updates to solve state estimation problems using first-order optimization methods (i.e., gradient descent methods), based on quadratic approximations of the original problem.

To promote \textit{physical} feasibility of the solution, many works impose equality or inequality system constraints by i) encoding hard constraints inside NN layers (e.g. using sigmoid layer to encode technical limits of upper and lower bounds), ii) applying prior on the NN architecture (e.g., Hamiltonian \cite{hamiltonianNN} and Lagrangian
neural networks \cite{lagrangianNN}), iii) augmenting the objective function with penalty terms in a supervised \cite{ppf-dnn} or unsupervised \cite{acopf-dnn-donti}\cite{pf-dnn-topo} way, iv) projecting outputs \cite{dcopf-dnn} to the feasible domain, or v) combining many different strategies. 
%In general, ML models with system characteristics taken into account are often named as \textit{model-based}, compared with a blind ML blackbox which is \textit{model-free}. 
In all these methods, incorporating (nonlinear) system constraints remains a challenge, even with state-of-the-art toolboxes \cite{neuromancer2022}, and most popular strategies lack rigorous guarantees of nonlinear constraint satisfaction. 

While these methods have advanced the state-of-the-art in physics-informed ML for power grid applications, critical limitations in terms of generalization, interpretation, and scalability exist. We discuss these further:

\textbf{Limited generalization:} Many existing methods do not adapt well to changing grid conditions. Take changes in network topology as an example. Many current works are built on non-graphical architectures without any topology-related inputs. These, once trained, only work for one fixed topology and cannot generalize to dynamic grid conditions. More recently, some works have begun to encode topology information. Graph model-based methods (e.g., GNN \cite{gnn-pf}\cite{gnn-acopf}\cite{gnn-se}) naturally impose topology as a hard constraint and thus can account for topology changes. Alternatively, work in \cite{pf-dnn-topo} encodes the topology information into the penalty term (as a soft constraint) through the admittance and adjacency matrix, and \cite{unrolled-gnu-se} accounts for topology in NN implicitly by applying a topology-based prior through a penalty term. While these methods lead to better topology adaptiveness, they also have some risks: the use of penalty terms \cite{pf-dnn-topo}\cite{unrolled-gnu-se} to embed topology information as a soft constraint can lead to limited precision; and, for problems (like OPF) where information needs to be exchanged between far-away graph locations, the use of GNNs requires carefully designed global context vectors to output predictions with global-level considerations. 
%Our paper designs a graph model based method that can exactly encode different topologies.

\textbf{Limited interpretability:} Despite that many ML models (NN, decision trees, K-nearest-neighbors) are universal approximators, interpretations of their functionality from a physically meaningful perspective are still very limited. The general field of \textit{model interpretability} \cite{interpretability} focuses on explaining \textit{how a model works}, to mitigate fears of the unknown.
Broadly, investigations of interpretability have been categorized into transparency (also called ad-hoc interpretations) and post-hoc interpretations. The former aims to elucidate the mechanism by which the ML \textit{blackbox} works before any training begins by considering the notions of \textit{simulatability} (Can a human work through the model from input to output, in reasonable time steps through every calculation required to
produce a prediction?), \textit{decomposability} (Can we attach an intuitive explanation to each part of a model: each input, parameter, and calculation?), and \textit{algorithmic transparency} (Does the learning algorithm itself confer guarantees on convergence, error surface even for unseen data/problems?). And \textit{post-hoc interpretation} aims to inspect a learned model after training by considering its natural language explanations, visualizations
of learned representations/models, or explanations of empirical
examples. However, none of these concepts in the field of ML model interpretability formally evaluates \textit{how a ML model makes predictions in a physically meaningful way} when it is used on an industrial system like the power grid.  Some recent works have explored the physical meaningfulness of their models from the power system perspective. Still, interpretations are made in conceptually different ways without uniform metric: Unrolled neural networks (which has been used as data-driven state estimation for power grid \cite{unrolled-gnu-se}\cite{unrolled-se-2018}) are more decomposable and interpretable in a way that the layers mimic the iterations in the physical solvers, yet these models \cite{unrolled-se}\cite{unrolled-se-2018}\cite{unrolled-gnu-se} mainly unroll first-order solvers instead of the second-order (Newton-Raphson) realistic solvers.
GNN-based models \cite{gnn-pf}\cite{gnn-acopf}\cite{gnn-se} naturally enable better interpretability in terms of representing the graph structure. 
Work in \cite{ppf-dnn} provides some interpretation of its DNN model for PF by matching the gradients with power sensitivities and subsequently accelerating the training by pruning out unimportant gradients. \cite{pf-dnn-topo} learns a weight matrix that can approximate the bus admittance matrix; however, with only limited precision. To summarize, due to the limited interpretability, ML models still have some opacity and blackbox-ness, when compared with the purely physics-based models (e.g., power flow equations).
%Our paper addresses this issue by defining a new concept \textit{physical interpretability}. 

\textbf{Scalability issues}:
In the case of large-scale systems, models (like DNNs) that learn the mapping from high-dimensional input-output pairs will inevitably require larger and deeper designs of model architecture and thereafter, massive data to learn such mappings. This can affect the practical use in real-world power grid analytics.
%This paper addresses these issues through a distributed scheme and the use of domain knowledge to regularize the model effectively.

\subsubsection{Anomaly detection and localization methods}

Beyond approximating simulators and state estimators, data-driven methods have been proved efficient in detecting and locating anomalies from data. Compared with bad data detection, anomaly detection presents a much stronger detectability to identify anomalous data, outages, and modern attacks, etc. A broad variety of machine learning techniques have been shown applicable to developing data-driven methods for this purpose, although with limitations in certain conditions. 

\textbf{Time Series Anomaly Detection:} 
Numerous univariate methods (hypothesis testings, auto-regressive and moving average models, etc.)  exist for anomaly detection in time series~\cite{keogh2007finding}. These methods apply to multivariate data when used together with dimension reduction techniques (principal component analysis, independent component analysis, etc.). Other methods have a multivariate nature and can learn spatial correlations in data.  Local outlier factor (LOF)~\cite{breunig2000lof} uses a local density approach. Isolation Forests~\cite{liu2008isolation}, as an ensemble method, partition the data using a set of trees for anomaly detection. Support vector machine (SVM) uses a classification method to make direct anomaly decisions.
More recently, many approaches use neural networks~\cite{yi2017grouped}, distance-based~\cite{ramaswamy2000efficient}, and exemplars~\cite{jones2014anomaly}. %However, they hardly consider the graph structure. 

\textbf{Anomaly Detection in Temporal Graphs:} \cite{akoglu2010oddball} found anomalous changes in graphs using an egonet (i.e. neighborhood) based approach, while \cite{chen2012community} uses a community-based approach. \cite{mongiovi2013netspot} found connected regions with high anomalousness. \cite{araujo2014com2} detected large and/or transient communities using Minimum Description Length. \cite{akoglu2010event} found change points in dynamic graphs, while other partition-based~\cite{aggarwal2011outlier} and sketch-based~\cite{ranshous2016scalable} works also exist for anomaly detection. However, these methods are not applicable to power grid anomaly detection because they focus on detecting unusual communities or connections, and power grid anomalies are detected from sensor data points.
%our approach has a very different goal of detecting disturbances which cause changes in sensor values. 

Most of these general-purpose techniques, however, suffer from a lack of domain knowledge, as they ignore the grid-specific temporal and spatial patterns. This can limit their practicality. The localization of anomaly sources can be rough and inaccurate without using accurate and complete system knowledge; e.g., without the knowledge of substation breaker configuration and its operation during a contingency, the fault on switching devices cannot be localized precisely.
Methods based on non-graphical models (e.g., auto-regressive models, neural networks) cannot consider network topology and can result in false positive outcomes when applied to a realistic dynamic graph. Also, neighborhood based methods significantly degrade in performance when faced with high-dimensionality which is common in power systems.

To address these limitations, many works have explored the inclusion of domain knowledge into machine learning. Attempts range from creating domain-knowledge-based features\cite{hooi2018gridwatch} and inserting domain knowledge into the models (e.g., topology information, network constraints, and technical limits), to building hybrid approaches that combine machine learning with physical solvers (e.g. building ML based warm starters). 

Chapter 3:

\section{A circuit viewpoint of simulation and estimation}
Power system has a circuit nature. Simulation \cite{SUGAR-pf-marko}\cite{SUGAR-pf}, estimation \cite{SUGAR-SE-Alex}\cite{SUGAR-SE-TnD}, and optimization \cite{SUGAR-opf} have been proved directly applicable to transmission and distribution grids without loss of generality, when we model power system as a circuit. However, today's industry standard formulations are not able to benefit from this generality. The transmission sector is widely modeled by 'PQV' formulation using non-linear power balance equations as shown in (\ref{eq:powerbalance}) and state variables $|V|, \theta$ under polar coordinate. Whereas, the distribution sector is widely modeled by current injection method, which is more aligned with circuit theory, with current balance equations written under rectangular coordinate. The distinct formulations prohibits us from being ready for the increasingly blurred boundary between transmission and distribution sectors induced by distributed energy resources; and also put obstacles in analyzing microgrids together with the main system. Table \ref{tab: PQV vs ECF} shows the difference between the two formulations:

\begin{table}[h]
\caption{Comparison between PQV and Circuit-based Formulation}
\label{tab: PQV vs ECF}
\begin{tabular}{c|c|c}
\hline
                     & \textbf{PQV Formulation}                                                                                                  & \textbf{Circuit-based Formulation}                                                                                          \\ \hline
Coordinate           & Polar coordinate                                                                                                          & Rectangular coordinate                                                                                                       \\ \hline
State variable       & \begin{tabular}[c]{@{}c@{}}Voltage magnitude and phase angle\\ $x=[|V_1|, \theta_1, ...., |V_N|, \theta_N]$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Real and imaginary voltage\\ $x=[V_1^R, V_1^I, ..., V_N^R, V_N^I]$\end{tabular}                 \\ \hline
Governing equations  & \begin{tabular}[c]{@{}c@{}}Nonlinear power balance equations\\ (active and reactive power balance) \\ See (\ref{eq:powerbalance})\end{tabular}    & \begin{tabular}[c]{@{}c@{}}Current balance equations  \\ by Kirchhoff's current law (KCL)  \\ See (\ref{eq: kcl example start})-(\ref{eq: kcl example end})\end{tabular} \\ \hline
Nonlinear components & \begin{tabular}[c]{@{}c@{}}Transmission lines and shunt elements \\ (leads to nonlinear power flow equations)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Generation (bus with PV control) \\ and Load (bus with PQ control)\end{tabular} \\ \hline
Linear components    & \begin{tabular}[c]{@{}c@{}}Slack bus, Load (bus with PQ control), \\ Generation (bus with PV control)\end{tabular}        & \begin{tabular}[c]{@{}c@{}}Slack bus, Transmission lines, and \\ Shunt elements (admittance)\end{tabular} \\ \hline
\end{tabular}
\end{table}


This thesis aims to further break the barrier in the context of situation awareness, building upon the existing works of equivalent circuit formulation for simulation and optimization purposes. In this chapter, we would like to start the road map from illustrate how a circuit viewpoint can provide  new insights into the efficiency and robustness of simulation and estimation problems; so as to inspire new opportunities for advancements.

Let us start from a toy example in Figure \ref{fig: ECF, case4}. In the left figure, a power system consists of generation units, loads, and branches (transmission lines or transformers) to deliver supply to load demands. Traditional RTU devices from the SCADA system and modern PMU devices are installed across the network to monitor the system in real time. 
\begin{figure}[h]
         \centering         \includegraphics[width=\linewidth]{figures/ckt-se/ECFidea-SnE.png}
         \caption{Circuit-based viewpoint for simulation and estimation on power system.}
         \label{fig: ECF, case4}
     \end{figure}

On a power system as such, models are established for each component, to represent either the fundamental laws that govern its behaviors or the observed behaviors at a certain time. These physical models enable numerical analysis like simulation and estimation:
\begin{itemize}
    \item For simulation, each power system component can be characterized (and numerically replaced) by a physics-behavior-based model. For steady-state analysis, a load is usually characterized by a static $PQ$ model; a generator is usually treated as a model with static power $P$ and voltage $|V|$ control.  Prior works \cite{SUGAR-pf}\cite{SUGAR-opf} have shown that each of the power system components (including constant power models, i.e. PQ and PV buses) can be directly mapped to an equivalent circuit model based on the underlying relationship between current and voltage state variables.
    \item For estimation, we propose that each measured the component can be characterized (and numerically replaced) by measurement-based models. The obtained measurement data represent certain constraints to describe an  operating point of the system. More specifically, consider a measurement of a generator's current to be the value of 1 per unit (p.u.), it represents a constraint that the generator is equivalent to some circuit element whose current equals 1 p.u., if the measurement is accurate. Then based on substitution theorem\cite{larry_book}, this generator can be equivalently replaced by an independent current source of 1 p.u., which is a linear equivalent circuit model of the measured generator. If we apply linear circuit modeling to every measured piece of equipment in the power system, we are able to map any measured power grid into corresponding circuit model. These models are flexible and can be added, removed or replaced to represent any changes on the system. Prior works \cite{SUGAR-SE-Alex} have made attempts to map a bus measured by PMU or RTU measurement devices into corresponding circuit elements. 
\end{itemize}

Following this idea, we can aggregate the component-wise models together, and represent the power system as a circuit system. As shown in the middle of Figure \ref{fig: ECF, case4}, both simulation and estimation tasks have similar objective of finding solutions to a feasible system:
\begin{itemize}
    \item Simulation: find state variables that can make this (circuit (a) in Figure \ref{fig: ECF, case4}) a feasible system that can deliver generation to load as pre-defined. In case of system collapse (i.e.,blackout), this (circuit system) becomes infeasible. 
    \item Estimation: find state variables that can make this (circuit (b) in Figure \ref{fig: ECF, case4}) a feasible system that is exactly consistent with what observed in data. In case of data errors, this (circuit system) becomes infeasible.
\end{itemize}


Let's first assume that a feasible system exist. Circuit-based modeling provides opportunities to advance efficiency of problem-solving. Decades of research in circuit simulation have developed mature heuristics\cite{sparsePFref15-spice} that can solve large-scale (nonlinear) circuit (with even billions of nodes) with fast speed. These heuristics includes but are not limited to variable limiting, homotopy methods, etc. For simulation problem, branches are linear with circuit-based formulation, so that nonlinearity only locally exists at bus locations of loads and generations. Prior works \cite{SUGAR-pf}\cite{SUGAR-pf}of circuit-based power flow analysis have successfully adopted these heuristics to simulate transmission and distribution systems. For estimation problem, apart from linear branch models and various heuristics, opportunities exist in improving linearity of the measurement-based models so that the entire circuit system can be highly linear. This thesis will develop measurement models to this end in Section \ref{sec: sugar meter models}, that can result in a completely linear circuit to represent the entire power system for highly-efficient steady-state estimation at a time $t$. 

Let's then discuss threat scenarios (e.g., blackout, measurement noises or errors) which makes the cases "infeasible". On a circuit system, these threats represent unwanted perturbations and spatial inconsistencies that make the circuit an infeasible system. How do we handle this? An immediate idea is to add compensations to make the network balance hold everywhere. On a circuit system, this can be easily implemented in the form of independent current sources, wherever a violation of nodal balance exist at a node (bus), we can add an independent current sources to make corrections and offset the discrepancy so that the circuit returns to a feasible system. If we can solve the system in a way to obtain optimal locations and values of these independent sources across the entire network, we get "threat indicators" for the system: 

\begin{itemize}
    \item For simulation, independent current source $n_i$ is a threat indicator of power deficiency at node location $i$. If we obtain optimal set of $n_1, n_2, ...$ for the entire system, we are informed of how severe the entire system blackout is and how much effort needed at each location to reconstruct a feasible system.
    \item For estimation, $n_{rtu}$ indicates the amount of noises at the RTU location, and serves to correctify the RTU measurement-based model so that it is consistent with measurements elsewhere. If we obtain optimal set of $n_{rtu}, n_{pmu}, ...$, we are informed of how noisy the data is, and get close to the true system which can generate the data as we observed.
\end{itemize}

% In the rest of the thesis, we will make various advancements in simulation and estimation tools, all of which will be inspired and implemented by circuit system. Table 
% compare notations?: The resulting mathematical formulation is defined on rectangular coordinate; I-V relationship are used to describe physics of an element; KCL equations are written at each node as network constraints


Clearly, this provides opportunities to build intrinsic robustness to simulation and estimation tools, because the threats can be captured and quantified with these threat indicators. To reveal the "optimal" values of these threat indicators,  simulation and estimation can be done equivalently on this circuit system, by formulating a constrained optimization problem under rectangular coordinate:
\begin{align}
    \min_{x,n} L(n)&\text{: a loss function to minimize threat indicators}\\
    \text{s.t.} H(x,n)=0&\text{: KCL equations of the 'circuit' system}
\end{align}

The level of robustness we can achieve depends highly on the choice of objective function. As previously defined in Problem \ref{def: sugar simulation}, minimizing the L2-norm (or weighted least squares) of threat indicators leads to converged simulation under blackout and severity quantified. This Chapter will extend the similar idea to estimation problem towards an convex and error-quantified estimation. Later Chapters will adopt new sparsity-encouraging objective functions to reach a higher level of robustness.

In the rest of this chapter, we focus on developing a circuit-based estimation that is highly efficient with its convexity and closed-form solution. First, Section \ref{sec: sugar meter models} will develop linear circuit models for all types of measurement devices. Then, Section \ref{sec: linear circuit and KCL} maps the power system into an aggregated equivalent circuit that can capture the system's stead-state operation point at the time of measurements; and shows that affine network constraints can be written. Next, Section \ref{sec: sugarSE} formulates an convex error-quantified circuit-based estimation problem, which proves to guarantee convexity and closed-form solutions. Its advantage over traditional estimation is discussed from both the optimization and probabilistic viewpoint in Section \ref{sec: sugar SE probabilistc view}.  Finally, Section \ref{sec: sugarSE result} demonstrates its advantage in speed by compare with traditional estimation method via experiments.
The estimation problems presented in this thesis have been also applied to combined transmission and distribution systems \cite{SUGAR-SE-TnD}. 

Chapter 4:
\section{Sparse optimization and robustness}

Sparse optimization is able to provide simple and structured vector or matrix values,  where most entries are zero, but only a few are non-zero.  This is usually achieved by either adding (L1) regularization or imposing additional constraints to encourage sparsity in the solution. 

The special structure of sparsity can be helpful and usually have intuitive meanings in engineering applications. 
For system control and optimization, we sometimes prefer easy actions taken at a few critical locations instead of all, which represents sparse recommendations. For signal processing, we might a selection of the most relevant features,  which represents a sparse recommendation or explanation. Moreover, when performing estimation or data processing problems, we are encountered with a sparse distribution of outliers or errors, which corresponds to a sparse explanation.  
Such kind of sparse recommendations and sparse explanations are ubiquitous to a real-world system.  A famous problem solving principle called Occam’s Razor stated that the simplest explanation is usually the best one.

Therefore, it becomes important to exploit sparse structures the analytical tools, in order to advance the robustness of these tools against the possibly "sparse" distribution of threats. Techniques to enforce sparsity been widely explored in literature. The LASSO method \cite{sparsePFref10-lasso} has been popular in explaining a signal as a sparse weighted sum of basis features. And weight least squared method have also been widely used for robust estimation\cite{robust-estimation-Huber}.  
The idea was first  introduced by Peter J. Huber\cite{robust-estimation-Huber}\cite{robust-regression-Huber} to apply L1 norm-based method as alternatives to least squares estimators for better handling outliers and non-Gaussian data distributions.

In this Section, we build on the existing tools in earlier Chapters to further advance their intrinsic robustness via sparse optimization. The key strategy is to exploit sparse structures in the "threat indicators" of circuit-based simulation and estimation problems. The resulting sparse threat indicators are able to pinpoint critical failure and error sources and make analytical tools immune to these threats. Figure \ref{fig: sparse error indicators} gives illustrative examples of our work. 

\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering         \includegraphics[width=0.8\textwidth]{figures/sparsePF/case14-1sparse.png}
         \caption{Simulation with sparse infeasibility indicators to pinpoint a dominant source of blackout: a sparse explanation of failure as well as sparse recommendation of fix.}
         \label{fig: wls bdd graph}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering         \includegraphics[width=0.95\textwidth]{figures/ckt-se/wlav_bdd_graph.png}
         \caption{Estimation with sparse error indicators to pinpoint 1 bad data and 2 topology errors: a sparse explanation of anomalous data.}
         \label{fig: wlav bdd graph}
     \end{subfigure}
     \caption{Toy examples: sparse optimization adding robustness to simulation and estimation}
        \label{fig: sparse error indicators}
 \end{figure*}

In the remainder of this Section, we first develop robust simulator by enforcing sparse infeasibility indicators in Section \ref{sec: sparsePF}; and then develop robust estimator by encouraging sparse error indicators in Section \ref{sec: ckt-GSE}.


Chapter 5:
\section{Temporal and spatial sparse structures for ML}

The previous Chapter \ref{ch: physics} has discussed the use of sparse optimization to bring intrinsic robustness into the simulation and estimation tools, producing sparse threat indicators to pinpoint failure sources and anomalies of interest. However, the modern threats are still not well handled in these physics-based simulation and estimation methods, leading to remaining gaps to be fulfilled. Below are two examples of remaining gaps:
\begin{itemize}
    \item Remaining efficiency gap: large-scale systems are hard to simulate due to the nonlinear nature of the power system simulation problem.
    \item Remaining robustness gap: existing analytical tools are not good at cyberthreats: estimation problems can be compromised by the anomalous injected by false data injection attack (FDIA)\cite{fdia-acse}\cite{fdia-review}; and simulation problems are not good at multiple-location disturbances like those induced by MadIoT attack \cite{madiot} because the simulator hardly has a initial condition close to the solution point when system changes significantly (this is also an efficiency gap)
\end{itemize}

These remaining gaps motivate the use of ML to predict and detect for under modern threats. 

In this Chapter, we highlight that the exploiting of sparse structures is helpful to develop simple-structured ML models with high-performance generalization and scalability. These ML models will contribute to situation awareness with advanced robustness and efficiency. 

We start from the discussing a temporal sparse structure. An important question ML often faces is: how to make a ML model generalize to (big) data that unavoidably come from different distributions? ML research is always struggling with bias and variance issues. Learning from too many irrelavant data can lead to high bias and even erroneous predictions, whereas not making use of the large data set can potentially cause high-variance (i.e., overfitting). 

\begin{figure}[h]
	\centering
\includegraphics[width=0.8\linewidth]{figures/dynwatch/sparse_and_generalization.png}
	\caption[]{Temporally sparse weights pinpoint the relevant historical data: a sparse recommendation.}
	\label{fig: temporal sparsity}
\end{figure}

Assigning sparse temporal weighting provides a solution to this issue, by giving sparse recommendation of relevant historical data. As shown in Figure \ref{fig: temporal sparsity}, suppose we need to make a data-driven prediction at time $t$, from historical data come from $K$ different distributions. Grouping these data into $K$ datasets, we can assume that each dataset is drawn from its corresponding distribution $N_k, \forall k=1,2,...,K$. Suppose the true distribution takes the form as shown in the figure. 
%Dataset 1 and dataset 3 are drawn from negatively centered distributions (marked in orange), whereas the distribution at $t$ is positively centered (marked in green). 
Dataset 1 and 3 are assigned with zero weights, since they are irrelevant data too far from the distribution at time $t$. Whereas, the remaining relevant datasets are assigned with non-zero weights.
%Dataset 2 is highly similar to the distribution at $t$, thus assigned with higher weight values. Dataset K is also weakly similar, thus assigned with lower weight values. 
Suppose we are able to optimally assign sparse weights reflecting the relevance of data; and make time $t$ predictions using weighted historical data. Then these sparse weights are able to pinpoint the the level of contribution each dataset should make in our final prediction for time $t$, and remove the irrelevant data that might cause a biased output. Section \ref{sec: dynwatch} will further elaborate on this idea, by developing \method, a distance-based method to obtain the sparse weight vector from an optimal bias-variance trade-off.

On the other hand, large power system is typically spatially sparse due to its sparse edge connections, i.e., each bus (node) is only connected to a few adjacent lines, instead of fully connected with all other nodes. This leads to highly sparsity of power system admittance matrix. \cite{Alvarado1976computation} shows that for typical power systems, a reasonable complexity of solving linear $Y_{bus}x=b$ is $n^{1.2}$. In Section \ref{sec: gridwarm}, we will develop exploit sparse graphical structures to design a "lightweight" ML predictor, which is simple-structured, but generalizable, scalable and interpretable.

Chapter 6:

\section{High-level idea of Physics-ML Synergy}

Despite the advances in existing approaches, there remain some tasks that are challenging and even impossible for state-of-the-art physics-based and data-driven approaches. 
A key challenge regarding efficiency is to make simulation both fast and accurate for a large-amount of scenarios and for hard-to-solve scenarios. 
A significant challenge regarding robustness is the mitigation of modern threats in the form of cyberattacks leveraging system physics. 
%Dynamic modeling provides defense against such cyberattacks, but is usually limited to short-term horizons (e.g., a few seconds), and models become highly complicated when the system is characterized by nonlinear differential equations.
State-of-the-art ML tools are successful in alarming these modern attacks, but they undesirably require human intervention to further mitigate these anomalies. This is because without the detailed physical model, even an advanced ML anomaly detector can only provide the alarm and a rough neighborhood indicating the suspicious anomalous region. Given that (state) estimation has been compromised, the true system state is hardly known, sometimes leaving it unknown what to follow from the current situation. This often necessitates human intervention in the anomaly mitigation process. 


%Moreover, using data-driven alternatives to replace model-driven tools in operation raises the concern of limited trustworthiness in safety-critical applications. This is induced by a variety of reasons, e.g., limited explainability, interpretability and the risk that ML may fail to generalize. One strategic method to improve is by enforcing physical constraints on the output space of ML models. Works in DC3,  \cite{DC3} and NeuroMANCER \cite{Neuromancer2023} \cite{DL-homotopy} have explored a strategic way of doing so.  They have highlighted the importance of providing guarantees of rigorously satisfying safety-related constraints, via regularization, projection, corrections, etc.   In a collaboration with PNNL (Pacific Northwest National Laboratory), we explored the use of homotopy-based meta-optimization heuristics to help with the model training. However, some models that use soft-constraints and not well-trained on heavily-constrained safety-critical still result in non-negligible constraint violations \cite{grid-reality}. \\

\begin{figure}[h]
     \centering
            \includegraphics[width=0.7\linewidth]{figures/SynSA-grid/synergy-idea.png}
    \caption{We advocate for a Physics-ML synergy: physics-based and data-driven models are interconnected to augment each other.
    }
    \label{fig: synergy concept}  
\end{figure}

Physics-based and data-driven approaches can be mutually complementary, motivating  Physics-ML Synergy framework in this thesis. In the remainder of this Chapter, we apply this high-level idea of synergy design in both simulation and estimation applications, advancing situation awareness through a collaborative architecture:
\begin{itemize}
    \item Section \ref{sec: synergy for simulation} develops Physics-ML Synergy for simulation via an interconnection of GridWarm ML predictor (Problem \ref{def: gridwarm} in Section \ref{sec: gridwarm}) and robust circuit-based simulator (Problem \ref{def: sparsePF simulation} in Section \ref{sec: sparsePF}. In this synergy, ML prediction is fed into physics-based simulator as warm starting point, while system knowledge and data are given to ML for learning of threat impact. The ultimate goal is to achieve both fast speed from ML and accuracy from physics-based simulator.
    \item Section \ref{sec: synergy for estimation} develops Physics-ML Synergy for estimation by interconnecting time-series ML \method (Problem \ref{def: dynwatch} in Section \ref{sec: dynwatch}) and robust circuit-based estimator (Problem \ref{def: ckt-GSE} in Section \ref{sec: ckt-GSE}). In this synergy, prior knowledge from ML comes in the form of regularization to augment estimation problem, and system knowledge is integrated into ML for predicting normal system behavior. The ultimate goal is to achieve a higher level of robustness to a mixture of tradtional and modern threats.
\end{itemize}

Conclusion:

This thesis resolves the grand challenge problem of improving situational awareness to make future electrical power grid and the broad class of related CPS infrastructures resilient and reliable.
To this end, this thesis made significant advancements in the state-of-the-art simulation and estimation tools which are key to situational awareness. The key contribution is the resolving of efficiency and robustness gaps which represent key obstacles to these tools. Within the scope of this thesis, we have focused on the steady-state power system and achieved fast speed on up to 80K-node network (the eastern interconnection); as well as a higher level of robustness that gives meaningful and actionable results under blackout failures, corrupted data, and a variety of cyberattack scenarios.

 
Towards making these achievements, this thesis first addressed the inherent limitations within physics-based and data-driven   categories (commonly used to design situational awareness tools). The key enablers in this part include using circuit-based formulation and exploiting sparse structures. And further, this thesis transcended the boundaries of conventional algorithmic design in the direction of a new hybrid paradigm: "Physics-ML Synergy", which draws on and combines the best of the two worlds. 

The chapters of this thesis were structured to form the different pieces of the complete "puzzle". 
First, Chapter \ref{ch: ECF} generalized the modeling of a steady-state power system into a circuit, with an extension from simulation to real-time estimation purposes. We discussed from a circuit viewpoint that both simulation and estimation problems can be treated as solving the feasible solution to a circuit system on which the device models of transmission lines, generators, loads and shunts are equivalent circuit elements. We also illustrated that, for simulation, these devices models come from system behaviors; whereas for estimation, device models can depend on real-time measurements. This Chapter further developed measurement-based device models with linear circuit modeling and demonstrated that circuit-based estimation for large-scale power systems can be formulated with inherent convexity, and solved with fast speed and scalability. This circuit approach addressed the inherent nonlinearity induced by traditional measurements and results in an efficient estimator applicable to combined transmission and distribution systems. 

Followed by the mapping of steady-state simulation and estimation to a circuit-solving problem, Chapter \ref{ch: physics} further introduced sparse optimization to bring intrinsic robustness into the methods. Intuitively, we look into system blackout and anomalous measurement data which lead to "infeasible circuit systems" (for simulation and estimation respectively). Independent current sources can be added to the circuit device models, restoring a feasible system, and serving as indicators of these threats. This Chapter developed sparse enforcing techniques towards formulating robust circuit-based simulation and robust circuit-based estimation problems. The result demonstrated that the resulting simulation produces sparse "infeasibility" indicators to pinpoint dominant sources of blackout and suggest actionable fix; similarly for estimation where our estimator produces sparse error indicators to identify and reject anomalous data. These methods solves efficiently on up to 80k-node network (the Eastern Interconnection power grid); and advanced the overall robustness of situational awareness, and enhanced decision-making to mitigate random threats.

With some intrinsic efficiency and robustness to random threats built within the physics-based simulation and estimation tools, the second piece of the puzzle is to leverage data-driven predictors and detectors to handle more advanced threats. It was illustrated that exploiting temporal and spatial sparse structures in the ML model design can contribute to lightweight ML methods which are simple-structured but scalable, generalizable and interpretable. In the first application, we exploit temporal sparse structure to develop \method, which is the first to adapt time-series anomaly detection to sensors placed on dynamic graphs in the context of large-scale electrical grids, and achieves real-time processing at the millisecond scale for 60K-node power systems (75\% the size of the Eastern Interconnection) per time tick per sensor. In the second application, we exploited spatial sparse graphcial structures towards developing GridWarm, a highly lightweight ML predicting threat impact.

Last but not least, after addressing the inherent limitations in both the physics and ML world, Chapter \ref{ch: synergy} completed the final piece of the puzzle - Physics-ML Synergy where physics-based tools “chat with” ML to merge their benefits. We show that interconnecting these tools makes a transformative impact to accomplish tasks that are impossible for each separate tool. In this thesis, it was demonstrated that interconnecting GridWarm predictor with circuit-based simulator, in the form of providing warm start points, leads to 3x faster simulation on hard-to-solve multiple-location load disturbances. And it was also shown that interconnecting \method prediction with robust circuit-based estimator, in the form of feeding prior knowledge, results in diminishing the impact of false data injection attack (a cyberattack) and accurately identifying a mixture of random anomalies and targeted cyberattack events. These efforts provides strong evidence to demonstrate that Physics-ML Synergy is able to bring the efficiency and robustness of situational awareness to the next level. 

For future works, we are seeing exciting opportunities of building on this prior foundation to extend Physics-ML Synergy designs for broad range of estimation, simulation, optimization, and defense applications. This opens room to explore how collaborative efforts from the two worlds can enable secure, time-efficient, and robust operation and planning, initially in the context of electric power systems but with broad generalizability to other smart infrastructure systems. The proposed research is both fundamental and potentially transformative in practice, given the rapid electrification to support decarbonization in many industries and connected infrastructures.

Specifically, one possible direction for Physics-ML Synergy research is to address more complex anomalies, threats and uncertainties that are occurring today.
In the energy sector, voltage spikes and transients are dynamic anomaly conditions that can malfunction the electric devices; vulnerabilities in modern power electronics expand the attack surface; renewable energy introduces more uncertainties and instabilities; and new cyberattacks (e.g., MadIoT, CrashOverride) and adversarial attacks motivate continuous improvements on the information security and model robustness. Physics-ML Synergy provides a new solution to these challenges, by adaptively interconnecting distinct modeling and data-driven components (each focusing on specific types of threats) so as to comprehensively address the diverse threats.

Another potential direction is the Physics-ML Synergy can leverage ML to complement for the missing physics in partially-known or paritially-observable scenarios. One notable example of partial-observability is the distribution power grids where some local regions are merely measured ``on the top", with limited or even no real-time information of what is happening inside. To handle partial observability, a lot of efforts in literature have been made on optimal sensor placement to make the system fully-observable \cite{sensor-placement}, learning the entire system through data-driven function approximators \cite{structure-learning}, as well as network tomography approaches to estimate hidden states from observations \cite{network-tomography}.
{Now Physics-ML Synergy provides a new possibility by investigating how ML can interconnect with physical tools to complement partial observability and derive something meaningful about the unobservable and unknown regions.}

Moreover, in the general field of engineering systems, future research also has the potential towards a strategic way and distributed implementation of Physics-ML Synergy. Based on user-defined physical models and ML, there potentially exists an optimal way of interconnecting these  tools to maximize the over performance for solving constrained optimization problems, system identification, simulation and problems for any given cyber-physical system.
Moreover, for systems that have a network nature, the implementation of Physics-ML Synergy can also be optimized to run in parallel via distributed computing. 
This includes developing a  federated distributed control scheme for components in the Physics-ML Synergy and their interconnections. 
As a result, a large-scale cyber-physical system can perform autonomous edge computing for local defense, simulation, and optimization within a small segment, while providing sufficient feedback information to the larger infrastructure for both spatial and time-based monitoring and analysis among these federated components.





